Search for a narrow charmed baryonic state decaying to D^*+/- p^-/+ in ep collisions at HERA

A resonance search has been made in the D^*+/- p^-/+ invariant-mass spectrum with the ZEUS detector at HERA using an integrated luminosity of 126 pb^-1. The decay channels D^*+ -> D^0 pi^+_s -> (K^- pi^+) pi^+_s and D^*+ -> D^0 pi^+_s -> (K^- pi^+ pi^+ pi^-) pi^+_s (and the corresponding antiparticle decays) were used to identify D^*+/- mesons. No resonance structure was observed in the D^*+/- p^-/+ mass spectrum from more than 60000 reconstructed D^*+/- mesons. The results are not compatible with a report of the H1 Collaboration of a charmed pentaquark, Theta^0_c.

==> com_def_tex/journal_def.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\em Nuovo Cimento}}
\def\NIM{{\em Nucl. Instrum. Methods}}
\def\NIMA{{\em Nucl. Instrum. Methods} A}
\def\NPA{{\em Nucl. Phys.} A}
\def\NPB{{\em Nucl. Phys.} B}
\def\PLB{{\em Phys. Lett.}  B}
\def\PR{{\em Phys. Reports} }
\def\PRA{{\em Phys. Reports}  A}
\def\PRL{{\em Phys. Rev. Lett.} }
\def\PRD{{\em Phys. Rev.} D}
\def\ZPC{{\em Z. Phys.} C}
\def\EPC{{\em Eur. Phys. J.} C}
\def\CPC{{\em Comp. Phys. Comm.} }
\def\CNPP{{\em Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\em Sov. J. Nucl. Phys.} }
\def\CJPB{{\em Czech. J. Phys.} B}
\def\IJMA{{\em Int. J. Mod. Phys.} A}
\def\RMP{{\em Rev. Mod. Phys.} }
\def\FP{{\em Fortschr. Phys.} }
\def\ZP{{\em Z. Phys.} }
%


==> com_def_tex/journal_def_foster.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\rm Nuovo Cimento}}
\def\NIM{{\rm Nucl. Instrum. Methods}}
\def\NIMA{{\rm Nucl. Instrum. Methods} A~}
\def\NPA{{\rm Nucl. Phys.} A~}
\def\NPB{{\rm Nucl. Phys.} B~}
\def\PLB{{\rm Phys. Lett.}  B~}
\def\PRA{{\rm Phys. Reports}  A~}
\def\PRL{{\rm Phys. Rev. Lett.} }
\def\PRD{{\rm Phys. Rev.} D~}
\def\ZPC{{\rm Z. Phys.} C~}
\def\EPC{{\rm Eur. Phys. J.} C~}
\def\CMC{{\rm Comp. Phys. Comm.} }
\def\CNPP{{\rm Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\rm Sov. J. Nucl. Phys.} }
\def\CJPB{{\rm Czech. J. Phys.} B~}
%


==> com_def_tex/newcom.tex <==
%
\newcommand{\GeVs}      {\mbox{${\rm GeV}^2$}}
\newcommand{\GeV}       {\mbox{${\rm GeV}$}}
\newcommand{\MeV}       {\mbox{${\rm MeV}$}}
\newcommand{\qsq}       {\mbox{${Q^2}$}}
\newcommand{\rhod}      {\mbox{${\rho^0}$}}
%\newcommand{\wgp}      {\mbox{${W_{\gamma p}}$}}
\newcommand{\wgp}       {\mbox{${W}$}}
\newcommand{\empz}      {\mbox{${\delta}$}}
\newcommand{\phid}      {\mbox{${\phi}$}}
\newcommand{\jpsid}     {\mbox{${J/\psi}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
%
\newcommand{\ys}        {\mbox{$y_{\Sigma}$}}
\newcommand{\xes}       {\mbox{$x_{e\Sigma}$}}
\newcommand{\wes}       {\mbox{$W_{e\Sigma}$}}
\newcommand{\eda}       {\mbox{$E_{DA}^{\prime}$}}
%
\newcommand{\ra}        {\mbox{$\rightarrow$}}
\newcommand{\gsp}       {\mbox{$\gamma^* p$}}
\newcommand{\xda}       {\mbox{$x_{DA}$}}
\newcommand{\qda}       {\mbox{$Q^{2}_{DA}$}}
\newcommand{\qe}        {\mbox{$Q^{2}_{e}$}}
\newcommand{\gsubh}     {\mbox{$\gamma_{_{H}}$}}
\newcommand{\te}        {\mbox{$\theta_{e}^{\prime}$}}
\newcommand{\Ee}        {\mbox{$E_{e}^{\prime}$}}
\newcommand{\gh}        {\mbox{$\gamma_{h}$}}
\newcommand{\mrsdm}     {\mbox{MRSD$_-^{\prime}$\ }}
\newcommand{\mrsdz}     {\mbox{MRSD$_0^{\prime}$\ }}
\newcommand{\ftwo}      {\mbox{$F_{2}$}}
\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c\bar c}$}}
%\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c}$}}
\newcommand{\ptr}       {\mbox{$p_{T}$}}
\newcommand{\ccb}       {\mbox{$c\bar{c}$}}
\newcommand{\dspm}      {\mbox{$D^{\ast \pm}$}}
\newcommand{\ds}        {\mbox{$D^{\ast}$}}
\newcommand{\dz}        {\mbox{$D^{0}$}}
\newcommand{\mc}        {\mbox{$m_{c}$}}
\newcommand{\dm}        {\mbox{$\Delta M$}}
\newcommand{\dsp}       {\mbox{$D^{\ast +}$}}
\newcommand{\xd}        {\mbox{$x(D^{\ast})$}}
\newcommand{\ptds}      {\mbox{$p_T(D^{\ast})$}}
\newcommand{\etads}     {\mbox{$\eta(D^{\ast})$}}
\newcommand{\mkpi}      {\mbox{$M_{K\pi}$}}
\newcommand{\mdz}       {\mbox{$M(D^0)$}}
\newcommand{\mkpipis}   {\mbox{$M_{K\pi\pi_{s}}$}}
\newcommand{\ps}        {\mbox{$\pi_{s}$}}
\newcommand{\sleq} {\raisebox{-.6ex}{${\textstyle\stackrel{<}{\sim}}$}}
\newcommand{\sgeq} {\raisebox{-.6ex}{${\textstyle\stackrel{>}{\sim}}$}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%


==> com_def_tex/physics_rus.tex <==
%
\newcommand{\rgevs}     {\mbox{$\,$Ĵ'$^2$}}
\newcommand{\rgev}      {\mbox{$\,$Ĵ'}}
\newcommand{\rmev}      {\mbox{$\,$δ'}}
%

